Before It's Too Late: A State Space Model for the Early Prediction of Misinformation and Disinformation Engagement

In today's digital age, conspiracies and information campaigns can emerge rapidly and erode social and democratic cohesion. While recent deep learning approaches have made progress in modeling engagement through language and propagation models, they struggle with irregularly sampled data and early trajectory assessment. We present IC-Mamba, a novel state space model that forecasts social media engagement by modeling interval-censored data with integrated temporal embeddings. Our model excels at predicting engagement patterns within the crucial first 15-30 minutes of posting (RMSE 0.118-0.143), enabling rapid assessment of content reach. By incorporating interval-censored modeling into the state space framework, IC-Mamba captures fine-grained temporal dynamics of engagement growth, achieving a 4.72% improvement over state-of-the-art across multiple engagement metrics (likes, shares, comments, and emojis). Our experiments demonstrate IC-Mamba's effectiveness in forecasting both post-level dynamics and broader narrative patterns (F1 0.508-0.751 for narrative-level predictions). The model maintains strong predictive performance across extended time horizons, successfully forecasting opinion-level engagement up to 28 days ahead using observation windows of 3-10 days. These capabilities enable earlier identification of potentially problematic content, providing crucial lead time for designing and implementing countermeasures. Code is available at: https://github.com/ltian678/ic-mamba. An interactive dashboard demonstrating our results is available at: https://ic-mamba.behavioral-ds.science.

==> sections/1-introduction-v1.tex <==
% !TeX root = ../camera.tex

\section{Introduction}

\textcolor{red}{Missing from intro:
\begin{itemize}
    \item a clear definition of \icmamba and its novelties (early on);
    \item a discussion of the engagement at the level of individual posts and opinions -- a definition of opinions.
\end{itemize}
}

\revMAR{I don't really like the structure of the intro. Shall we try something along the following:
\begin{itemize}
  \item PARA1: Online social media can spread harmful content -- like mis and disinfo, what are each? --, but engagement with such content can vary wildly (from a lot to none, can we get some references of papers that study this in the social science?). This paper aims to forecast early the future engagement that mis and disinformation will get.
  \item PARA2: What engagement and what data sources? introduce the three levels of engagement, say that views are rarely captured and observed (unless you are the post's owner), but one-click engagements and comments are typically publicly visible as they drive the digital word-of-mouth process. Here, we use the CrowdTangle that give us interval-censored versions of these engagement measures such as in \cref{fig:sample_ic_mamba}
  \item PARA3: a short overview of approaches to forecast engagement metrics -- a summary of the two paragraphs that I labeled as belonging to the related works.
  \item CONTRIBUTIONS: @lin: I wonder if the Research questions are not a bit too narrow and too technical. With an intro as per the above, we would need something like: "Can engagement be predicted early?".
\end{itemize}
}


\begin{figure}[tbp]
  \centering
  \includegraphics[width=\linewidth]{images/sample_v9.pdf}
  \caption{
  \replace{
    Illustration of interval-censored social media engagement data. Following a post's creation at $t_0$, users perform engagement actions (view, like, comment, share, emoji) at timestamps $s_1$ through $s_8$. While individual actions occur continuously, engagement data is only collected at discrete observation points $t_j$, where each engagement vector $e_j$ captures the cumulative counts of different interaction types over intervals of length $\Delta t_j = t_{j+1} - t_j$.}{}
    \TODO{MAR}{Needs updating, need to describe what \mbox{$T_i$} are -- that is the unobserved exact times of engagements.}
  }
  \label{fig:sample_ic_mamba}
  \Description{social engagement matters sample}
\end{figure}


Social media platforms accelerate the spread of harmful content, particularly misinformation (false information shared without intent to harm) and disinformation (deliberately created and shared false information)~\citep{lazer2018science,scheufele2019science}. Large-scale analysis of social media cascades reveal extreme variations in engagement patterns -- while the most viral false news stories reach up to 100,000 users within hours, real-world browsing data shows that over 70\% of users never engage with such content, and a mere 0.15\% of users drive over 80\% of engagement~\citep{vosoughi2018spread, grinberg2019fake,guess2020exposure}. These findings highlight the critical role of early engagement patterns in determining content virality. Understanding and predicting these patterns early could enable platforms to identify potentially harmful content before it reaches viral scale, enabling proactive rather than reactive intervention strategies.

In this work, we aim to predict social media engagement patterns at both individual and collective levels. In the context of misinformation, individual posts express specific viewpoints or claims, while disinformation often manifests as coordinated narratives - broader storylines that emerge when multiple posts promote similar false claims~\citep{del2016spreading,vosoughi2018spread}. These narratives can spread rapidly across platform communities and even across different platforms~\citep{wilson2020cross}, making it crucial to predict not only individual post engagement but also the collective engagement patterns of posts sharing similar narratives~\citep{bak2021stewardship}. This multi-level prediction enables better early detection and proactive intervention strategies for both organic misinformation spread and coordinated disinformation campaigns.

Based on studies of user behavior and cognitive investment~\citep{lorenz2011social,mosleh2021cognitive,pennycook2021shifting,brady2021social}, we formalize engagement through a three-level hierarchy: views represent the most passive form of engagement and are typically only visible to content owners and platform operators; one-click engagements (likes, shares, and reactions) represent quick evaluative responses; while comments require users to formulate and articulate their thoughts. This hierarchical structure of engagement presents unique challenges for temporal prediction, particularly when modeling the interplay between different engagement types over time.

Our analysis leverages CrowdTangle data\footnote{\url{https://www.crowdtangle.com/}}, which has interval-censored engagement metrics, where observations are made at discrete time points ($t_0, t_1, ...$) with engagement counts recorded for each interval $\Delta t_j$ (as illustrated in \cref{fig:sample_ic_mamba}). For instance, within an interval $\Delta t_2$, we observed two likes, two shares, and two emoji reactions since the last observation, but not the exact timing of individual engagement events (e.g.\ $s_4$). As illustrated in \cref{fig:sample_ic_mamba}, engagement data is collected at discrete observation points $t_j$, where each engagement vector $e_j$ captures the cumulative counts of different interaction types over intervals of length $\Delta t_j = t_{j+1} - t_j$. This censored view of engagement progression, combined with the hierarchical nature of user cognitive investment, presents unique modeling challenges that reflect real-world platform constraints.

Recent deep learning approaches have made progresses in modeling social media engagement through different architectural innovations: language models for capturing coordinated posting behaviours~\citep{atanasov2019predicting,tian2023metatroll} and propagation models for modeling information diffusion~\citep{zannettou2019disinformation,im2020still,luceri2024unmasking,kong2023interval}. State space models have also demonstrated strong performance on sequential prediction tasks ~\citep{mamba,mamba2}, with their latent state representations theoretically well-suited for temporal dependencies. However, these approaches face two key limitations when applied to mis/disinformation engagement forecasting: (1) they primarily focus on classification tasks rather than quantifying future temporal patterns of engagement, and (2) they struggle with the irregularly sampled and bursty nature of viral content progression.

%In the digital age, social media platforms have become powerful tools for information dissemination, significantly influencing public opinion and societal dynamics. While these platforms facilitate rapid communication and information sharing, they also present challenges in the form of misinformation, disinformation, and state-backed influence operations. The spread of such content can have far-reaching consequences, potentially undermining social cohesion, public health, and even democratic processes~\citep{starbird2019disinformation,vosoughi2018spread,bradshaw2019global}.


%The detection of coordinated state-backed influence campaigns presents unique challenges. These operations leverage networks to sway public opinion and exacerbate social divisions~\citep{starbird2019disinformation}, with impacts ranging from eroding institutional trust to inciting violence~\citep{woolley2018computational}. Traditional approaches to this problem have relied on manual analysis by experts, which cannot scale with the volume and velocity of social media content~\citep{qiu2018deepinf,lazer2018science,sharma2019combating,allcott2017social}.

%We propose a hierarchical structure of social media engagement that reflects increasing levels of cognitive and temporal commitment from users, as shown on the right of \cref{fig:sample_ic_mamba}. Views are the most passive level of interaction, as they require minimal cognitive effort. The second tier is one-click engagement, which includes shares, likes and emoji reactions (e.g.\ angry or smile face). This is a low-threshold active interaction demonstrating a basic emotional or reactive response to the source. The highest level of user engagement is comments. It demands a larger time investment and requires users to formulate thoughts, compose language and consider social context.

%Recent deep learning approaches have advanced the detection of social media harmful content. 
%Transformer architectures capture coordinated posting behaviours~\citep{atanasov2019predicting}, while graph neural networks model information diffusion patterns~\citep{zannettou2019disinformation}. 
%Temporal modeling using RNNs and LSTMs has shown their abilities in modeling engagement dynamics~\citep{im2020still}. 
%However, these methods largely focus on binary detection of mis/disinformation, rather than quantifying their societal impact and influence. 
%In addition, they struggle to handle the inherent temporal and hierarchical complexities of social media engagement, particularly with irregularly sampled data and dynamic intervals between viral events.\mar{This para reads like literature review. Shuold not be in intro in this detail.}


%State space models have showed their capacities on language modeling~\citep{mamba,mamba2} and sequential prediction tasks~\citep{rangapuram2018deep}. 
%Their ability to model latent states aligns with capturing temporal dependencies and hierarchical relationships in sequential data. However, when applied to social media influence operations, state space models face limitations in handling the dynamic nature of engagement patterns. They struggle with irregular sampling intervals between viral events, variable engagement rates across different narratives, and the bursty nature of coordinated amplification campaigns. Additionally, they lack mechanisms to capture the hierarchical relationships between individual posts and broader narrative impact.\mar{Also reads as lit review.}

%Social media influence operations present increasingly complex challenges for detection and impact assessment, characterised by irregular viral events, coordinated amplification campaigns, and multi-level narrative structures. 


\boldsubtitle{Our contributions:}
We introduce \icmamba (Interval-Censored Mamba), a novel framework that integrates interval-censored data modeling with state space architecture to capture irregular temporal dynamics and predict engagement patterns across multiple granularities, from individual posts to broader narrative impact.
The paper addresses the following three Research Questions (RQs):

RQ1: \textit{How effectively can state space architectures model the temporal dynamics of interval-censored engagement data?}: IC-Mamba explicitly handles the irregular sampling and censored observations inherent in social media engagement data with time-aware positional embedding and interval-censor state representation. Our experiments demonstrate a 4.72\% improvement in prediction accuracy compared to traditional methods, maintaining robust performance (RMSE 0.118-0.143) across diverse real-world datasets.

RQ2:\textit{ Can we forecast future engagement patterns early enough to enable proactive intervention?}: Through our experiments, we demonstrate \icmamba's capability to predict engagement metrics at multiple granularities, outperforming baselines by achieving lower RMSE at early prediction windows (15-30 minutes post-posting) and maintaining strong performance up to 3 hours. Our model can also captures both individual post dynamics (RMSE 0.118-0.143 across datasets) and group-level engagement patterns (F1 0.508-0.751 for narrative-level predictions).

RQ3: \textit{How effectively can we track and predict the long-term spread of opinions across social media platforms?}: Our experiments demonstrate the model's ability to forecast opinion-level engagement dynamics over extended periods, using observation windows of 3, 7, and 10 days to predict spreading patterns up to 28 days ahead. The results in \cref{fig:dynamic_pred} show IC-Mamba's effectiveness in capturing long-term opinion proliferation and evolution.

\icmamba is not intended to replace human expertise but rather to serve as a powerful tool to augment and streamline the work of social scientists and content moderators. By providing accurate, early predictions of content engagement and capturing complex temporal dynamics, our framework can help researchers identify potentially harmful information campaigns in their nascent stages, allowing for more timely and effective interventions.

==> sections/1-introduction-v2.tex <==
% !TeX root = ../camera.tex

\section{Introduction}

\begin{figure}[tbp]
  \centering
  \includegraphics[width=\linewidth]{images/sample_v9.pdf}
  \caption{
    Illustration of interval-censored social media engagement data. Following a post's creation at $t_0$, users perform engagement actions (view, like, comment, share, emoji) at timestamps $s_1$ through $s_8$. While individual actions occur continuously, engagement data is only collected at discrete observation points $t_j$, where each engagement vector $e_j$ captures the cumulative counts of different interaction types over intervals of length $\Delta t_j = t_{j+1} - t_j$.
  }
  \label{fig:sample_ic_mamba}
  \Description{social engagement matters sample}
\end{figure}


On 28 October 2017, an anonymous 4chan user made a brief yet impactful post on the platform claiming that Hillary Clinton was to be arrested in the coming days.\footnote{\url{https://www.bellingcat.com/news/americas/2021/01/07/the-making-of-qanon-a-crowdsourced-conspiracy/}}
On 6 January 2021, devotees of then-outgoing President Donald Trump stormed the United States Capitol building in an act of domestic terrorism designed to prevent President-elect Joe Biden's election victory from being confirmed. Five people died during and in the immediate aftermath of the attack, and an additional four died in the subsequent months \footnote{\url{https://www.factcheck.org/2021/11/how-many-died-as-a-result-of-capitol-riot/}}; and over 140 police officers were injured \footnote{\url{https://www.nytimes.com/2021/08/03/us/politics/capitol-riot-officers-honored.htm}}. 
Investigations by the Associated Press of the online social media profiles of over 120 of the rioters revealed high levels of adherence to the QAnon conspiracy theory that had begun just four years prior on 4chan.\footnote{\url{https://apnews.com/article/us-capitol-trump-supporters-1806ea8dc15a2c04f2a68acd6b55cace}}
Numerous explanations for the conspiracy's influence have been proposed, including its religious qualities~\citep{macmillen2022qanon}, its narrative and gaming attributes~\citep{haiven2022interview}, its inflammatory political and social values and its ability to quell uncertainty~\citep{young2022authoritarian}.
Given its ongoing impacts, the question must be asked: what if we could have seen this coming? More specifically, what if it had been possible to forecast the user engagement with this one 4chan account's postings and the fringe ideology that would morph into QAnon? Would we have been able to implement interventions to prevent these tragic outcomes?


We tackle the former question above and introduce \icmamba, a model capable of forecasting user engagement with online content. We go beyond the level of atomic posts to forecast the number of likes, shares, emoji reactions, and comments for ``emerging opinions'' – particular worldviews supported across a series of posts.
Our framework can forecast the arrival rate of posts supporting an opinion, and forecast the engagement for each, obtaining estimates of the total level of engagement for the entire opinion.
Our analysis leverages CrowdTangle data\footnote{\url{https://www.crowdtangle.com/}} with interval-censored engagement metrics, where observations are made at discrete time points with engagement counts recorded for each interval (as seen in \cref{fig:sample_ic_mamba}).

Recent deep learning approaches have made progress in modeling social media engagement through different architectural innovations: language models to capture coordinated posting behaviors~\citep{atanasov2019predicting,tian2023metatroll} and propagation models to model information diffusion~\citep{zannettou2019disinformation,im2020still,luceri2024unmasking,kong2023interval}. State space models have also demonstrated strong performance on sequential prediction tasks ~\citep{mamba,mamba2}, with their latent state representations theoretically well suited for temporal dependencies. However, these approaches face two key limitations when applied to mis/disinformation engagement forecasting: (1) they primarily focus on classification tasks rather than quantifying future temporal patterns of engagement, and (2) they struggle with the irregularly sampled nature of viral content progression.


\noindent\textbf{Our main contributions} address three research questions (RQs) at the intersection of temporal modeling and social media dynamics:

RQ1: \textit{How can we effectively model irregular temporal patterns in social media engagement?}: Through IC-Mamba's time-aware embeddings and state space model architecture, we capture the dynamics of online interactions, achieving a 4.72\% improvement over the state-of-the-art approaches. 

RQ2:\textit{Can we predict viral potential within the critical early window? }: \icmamba shows strong performance in the crucial 15-30 minute post-publication window (RMSE 0.118-0.143), while capturing both granular post-level dynamics and broader narrative patterns (F1 0.508-0.751 for narrative-level predictions).

RQ3: \textit{How effectively can we forecast the evolution of broader opinions?}: Our experiments demonstrate the model's ability to forecast opinion-level engagement dynamics over extended periods, using observation windows of 3, 7, and 10 days to predict spreading patterns up to 28 days ahead. \cref{fig:dynamic_pred} shows \icmamba's effectiveness in capturing long-term opinion proliferation and evolution.

As a tool, \icmamba streamlines the work of human experts, enabling earlier identification of problematic content, and therefore, providing more time to design and implement countermeasures.

==> sections/2-related-works.tex <==
% !TeX root = ../camera.tex

  

\section{Related Work}
This section reviews relevant literature in two key areas that underpin our approach to modeling and predicting social engagements during outbreak events such as information operations and natural disasters like the infamous 2019-2020 Australian Bushfires:
popularity and engagement prediction on social media platforms, and
state space models for sequence modeling and prediction.


%Comment out this part for now
%\subsection{Social Engagement Analysis}
%Social media platforms have become vital channels for disseminating information and engaging the public during crises, sparking significant research into online behavior patterns. 
%\citet{imran2015processing} conducted a thorough survey on social media use in emergencies, highlighting distinct patterns in information sharing and user interaction across various crisis types. 
%Building on this, \citet{stieglitz2018social} proposed a framework to track engagement metrics during crises, identifying key information sources and mapping the spread of crisis-related content.
%
%In the context of natural disasters, \citet{kryvasheyeu2016rapid} examined social media activity during Hurricane Sandy, uncovering correlations between public sentiment, engagement levels, and the hurricane's impact. Advances in predictive modeling have further expanded the field. For example, \citet{yin2012using} applied machine learning techniques to social media data, demonstrating their utility for enhancing situational awareness during emergencies. Similarly, \citet{cinelli2020covid} analyzed the dissemination of COVID-19 content across social platforms, offering valuable insights into information spread during public health crises.
%
%The challenge of differentiating organic engagement from manipulated activity has also gained prominence. 
%\citet{starbird2019disinformation} explored the proliferation of disinformation during crises, using network and content analyses to identify campaigns exploiting these events. 
%Their findings highlighted the intricate interplay between authentic public discourse and strategic information operations in high-stakes scenarios.

%The reviewed studies underscore social media engagement as a critical lens for understanding crisis responses, spanning natural disasters, pandemics, and disinformation campaigns. 
%However, they primarily treat engagement as an external signal without modeling its temporally dynamic and complex nature during outbreak events. 
%This paper advances online engagement modeling and prediction by addressing key challenges, including handling irregular time intervals, capturing both granular and aggregate trends, and adapting to rapidly evolving social landscapes.

\begin{table}[t]
    \caption{
    Information used in related studies and our work (\icmamba). V: views, S: shares/retweets, 
    C: comments, L: likes, E: emojis, WB: Weibo, YT: Youtube, FB: Facebook.
    }
    \label{tab:related_work}
    %\begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{lcccccc}
    \toprule
    &V &S & C & L & E & platform \\ \toprule
    DeepCas~\citep{li2017deepcas} & &\checkmark & & & & X\\
    DeepHawkes~\citep{cao2017deephawkes} & &\checkmark & & & &X \\
    Topo-LSTM~\citep{wang2017topological} & &\checkmark & & & &X \\
    HIP ~\citep{rizoiu2017expecting} &\checkmark &\checkmark & & & &YT \\
    DeepInf~\citep{qiu2018deepinf} & &\checkmark & &\checkmark & &WB and X \\
    B-Views~\cite{wu2018beyond} &\checkmark & & & & & YT \\
    SNPP ~\citep{ding2019social} & & & &\checkmark & &X \\
    CasFlow~\citep{xu2021casflow} & &\checkmark & & & &WB \\ 
    %DUMMY~\cite{wu2018beyond} &\checkmark & & & & & Youtube \\
    MBPP~\cite{rizoiu2022interval} &\checkmark &\checkmark & & & &YT \\
    %PCMHP~\citep{xu2021casflow} & &\checkmark & & & &WB \\
    IC-TH~\cite{kong2023interval} & &\checkmark & & & &X \\
    OMM~\citep{calderon2024opinion} & &\checkmark & & & &X,YT\& FB \\
    %Hawkes Mixture Model~\citep{xu2021casflow} & &\checkmark & & & &WB \\
    \midrule
    \icmamba & &\checkmark &\checkmark & \checkmark &\checkmark & FB \\
    \bottomrule
    \end{tabular}
    %\end{adjustbox}
\end{table}

\subsection{Popularity and Engagement Prediction}
Social media engagement prediction research spans various platforms and prediction tasks. 
DeepCas~\citep{li2017deepcas} used random walk and attention mechanisms to predict final cascade size on X, while SNPP~\citep{ding2019social} applied temporal point process with a gated recurrent unit architecture for tweet repost count prediction.
Topo-LSTM~\citep{wang2017topological} incorporated user interaction sequences through a topological structure for retweet prediction, while DeepInf~\citep{qiu2018deepinf} on Weibo and X predicted user retweets, likes, and following behaviors using graph convolutional networks within the 2-hop neighborhood. 
CasFlow~\citep{xu2021casflow} used hierarchical attention networks for modeling Weibo reposts.
Several approaches have focused on handling temporal dynamics in engagement prediction. DeepHawkes~\citep{cao2017deephawkes} integrated reinforcement learning with Hawkes processes for retweet cascade prediction.
For YouTube, HIP~\citep{rizoiu2017expecting} and MBPP~\citep{rizoiu2022interval} advanced temporal modeling for views prediction, with B-Views~\citep{wu2018beyond} specifically addressing cold-start scenarios.
Recently, IC-TH~\citep{kong2023interval} tackled the challenge of incomplete observations in retweet prediction on X, while OMM~\citep{calderon2024opinion} proposed a mathematical framework for shares prediction on X, YouTube, and Facebook.
While these approaches have advanced cascade modeling, existing interval-censored methods (IC-TH, MBPP) focus on single-post dynamics without considering broader opinion-level patterns. Our work extends beyond individual post predictions to model collective opinion engagement on Facebook, and we include these interval-censored models along with neural approaches (TH~\cite{zuo2020transformer}) as baselines.

%comment out this part for now.
%\subsection{Information Operation}
%Information operations on social media platforms have become a significant concern for researchers and policymakers alike. \citet{bradshaw2018global} conducted a study on the global organisation of social media manipulation, revealing the widespread use of computational propaganda by governments and political parties. It highlighted the scale and sophistication of modern information operations.
%The detection of information operations has been a key focus area. \citet{varol2017online} developed machine learning techniques to identify social bots.
%In the context of political influence, \citet{allcott2017social} analysed the impact of fake news during the 2016 U.S. presidential election, quantifying its reach and potential effects on voter behaviour. It showed the need for robust methodologies to measure the real-world impact of online disinformation campaigns.
%Recent advancements have focused on cross-platform analysis of information operations. \citet{zannettou2018origins} traced the spread of memes across multiple social media platforms, revealing how coordinated campaigns exploit different platform characteristics to maximise their reach and impact.

%While existing studies have made progress in detecting and analysing such operations, they often fall short in forecasting their potential reach and impact. The ability to accurately predict the influence of information operations on social media is crucial for developing proactive mitigation strategies and understanding their evolving dynamics. 


\subsection{State Space Model in Sequence Modeling}
State Space Models (SSMs) have recently emerged as a robust alternative to traditional sequence modeling approaches, particularly for capturing long-range dependencies. 
In sequence modeling applications, \citet{hasani2021liquid} demonstrated the effectiveness of continuous-time neural networks based on SSMs for time series forecasting in healthcare, while \citet{rangapuram2018deep} explored deep-state space models for time series forecasting.

\citet{gu2022efficiently} introduced the structured state space sequence model, demonstrating its efficiency in processing sequences of up to a million steps.
Building on this, \citet{dao2022flashattention} developed a hybrid approach combining SSMs with selective attention mechanisms, achieving competitive performance on language modeling benchmarks while maintaining computational efficiency.
Recent work introduced a selective state space model that achieved state-of-the-art performance while preserving linear time complexity, demonstrating that SSMs could match or exceed transformer-based architectures in language modeling tasks~\citep{mamba,mamba2}. 

Despite these advancements, few studies have applied modern SSM architectures to predict or analyze social media engagement, particularly in the context of disinformation campaigns or crisis events. 
Our work bridges this gap by extending the Mamba architecture to handle non-uniform intervals, while identifying misinformation opinions and disinformation narratives.
%This paper introduces \icmamba, an online attention modeling and prediction tool that extends the Mamba architecture in several ways. 
%\icmamba handles interval-censored data with non-uniform intervals, identifies misinformation opinions and disinformation narratives.







==> sections/fig-4-data-single.tex <==
% !TeX root = ../camera.tex

\begin{figure}[t]
    \centering
    \newcommand\myheight{0.135}
    {
        \includegraphics[height=\myheight\textheight]{images/eccdf_social_media_comments_2021_v4.pdf}
        \label{fig:data_insights_comments}
    }%
    \caption{ Temporal evolution of comment distributions across different time windows ranging from 1 hour to 7 days, demonstrating the dynamic patterns of social media engagement over time. Note: ECCDF represents Empirical Complementary Cumulative Distribution Functions.}
    \label{fig:data_insights}
\end{figure}
